Methods to Estimate Cryptic Sequence Complexity

Complexity is a signature quality of interest in artificial life systems. Alongside other dimensions of assessment, it is common to quantify genome sites that contribute to fitness as a complexity measure. However, limitations to the sensitivity of fitness assays in models with implicit replication criteria involving rich biotic interactions introduce the possibility of difficult-to-detect ``cryptic'' adaptive sites, which contribute small fitness effects below the threshold of individual detectability or involve epistatic redundancies. Here, we propose three knockout-based assay procedures designed to quantify cryptic adaptive sites within digital genomes. We report initial tests of these methods on a simple genome model with explicitly configured site fitness effects. In these limited tests, estimation results reflect ground truth cryptic sequence complexities well. Presented work provides initial steps toward development of new methods and software tools that improve the resolution, rigor, and tractability of complexity analyses across alife systems, particularly those requiring expensive in situ assessments of organism fitness.

==> Dockerfile <==
FROM mmore500/docker-texlive-full:sha-ea45eb5

COPY . /opt/cryptic-sequence-concept/tex

SHELL ["/bin/bash", "-c"]

# Define default working directory.
WORKDIR /opt/cryptic-sequence-concept/tex

# Prevent interactive time zone config.
# adapted from https://askubuntu.com/a/1013396
ENV DEBIAN_FRONTEND=noninteractive

RUN \
  echo 'Acquire::http::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::ftp::Timeout "60";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo 'Acquire::Retries "100";' >> "/etc/apt/apt.conf.d/99timeout" \
    && \
  echo "buffed apt-get resiliency"

RUN \
  find /etc/apt -type f -name '*.list' -exec sed -i 's/\(^deb.*-backports.*\)/#\1/; s/\(^deb.*-updates.*\)/#\1/; s/\(^deb.*-proposed.*\)/#\1/; s/\(^deb.*-security.*\)/#\1/' {} + \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  echo "removed -backports, -updates, -proposed, -security repositories"

# magic to fix java installation conflict in subsequent apt install
# see https://github.com/geerlingguy/ansible-role-java/issues/64
RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    man \
    && \
  rm -rf /var/lib/apt/lists/* \
    && \
  mkdir /usr/share/man/man1/

RUN \
  apt-get update -q --allow-unauthenticated \
    && \
  apt-get install -qy --no-install-recommends \
    bibtool \
    git \
    make \
    moreutils \
    nodejs \
    pcregrep \
    pdftk \
    && \
  rm -rf /var/lib/apt/lists/*

CMD ["bash"]


==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := $(shell basename $(abspath $(dir $(lastword $(MAKEFILE_LIST)))/..))

DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh


==> draft.tex <==
\def\mydraft{
\usepackage{draftwatermark}
\usepackage{lineno}
\linenumbers
\renewcommand{\linenumberfont}{\normalfont\small\color{red}}
}
\input{main.tex}


==> lib/dissertationexclude.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationexclude}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION
\else
#1
\fi
}


==> lib/dissertationonly.tex <==
\pragmaonce

% adapted from https://www.overleaf.com/learn/latex/Commands
\newcommand{\dissertationonly}[1]{%
% adapted from https://tex.stackexchange.com/a/33577
\ifdefined\DISSERTATION%
#1%
\else%
\fi
asdf
}


==> lib/importpath.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \def\importpath{\import@path}
\makeatother


==> lib/safepercent.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\newcommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\newcommand\safetilde{\string~}


==> text/body/methods.tex <==
\section{Methods} \label{sec:methods}

% For initial tests of proposed, we used a simple genome model where sites had explicitly ascribed effects.
% This allowed us to design trials with known effects in genomes and then assess the capability assays to recover this information.
% Effects were assigned randomly, to genome sites and multiple effects were allowed to overlap on the same site.
% When evaluating the knockout effects on a genome, we summed constituent effects and defined a deleterious outcome if these effects summed to a value greater than 1.0.
% Additive sites contributed a constant amount TODOAMOUNT to the sum if knocked out.
% Epistatic sites are created in sets of TODOAMOUNT sites, and an effect of TODO was only accured if all sites in a set were knocked out.

